Feedback cooling of atomic motion in cavity QED

We consider the problem of controlling the motion of an atom trapped in an optical cavity using continuous feedback. In order to realize such a scheme experimentally, one must be able to perform state estimation of the atomic motion in real time. While in theory this estimate may be provided by a stochastic master equation describing the full dynamics of the observed system, integrating this equation in real time is impractical. Here we derive an approximate estimation equation for this purpose, and use it as a drive in a feedback algorithm designed to cool the motion of the atom. We examine the effectiveness of such a procedure using full simulations of the cavity QED system, including the quantized motion of the atom in one dimension.

==> makedoc <==
#!/bin/sh

rm *.ps *.eps *.png *.bbl *.dvi *.blg *.aux *.log *.tex *.bib *.pdf

cp ../traj18_layoutrbgln.eps fig1.eps
cp ../basic_coolingr_mod.eps fig2.eps
cp ../initcond_checkr_mod.eps fig3.eps
cp ../basic_directcoolingr_mod.eps fig4.eps
cp ../parity_squish_layoutr.eps fig5.eps
cp ../band_pops_layoutr.eps fig6.eps
cp ../epsilonsweep_layoutr.eps fig7.eps
cp ../vmaxsweep_theoryr.eps fig8.eps
cp ../gammasweep_theoryr.eps fig9.eps
cp ../epsilonsweepctr_layoutr.eps fig10.eps
cp ../band_pop_traj_layoutr.eps fig11.eps
cp ../smcavtest_mod.eps fig12.eps # was fig16.eps
cp ../longrun_mod.eps fig13.eps # was fig17.eps
cp ../etasweepr.eps fig14.eps # was fig12.eps
cp ../delaysweepr_mod.eps fig15.eps # was fig13.eps
cp ../updatesweepr_mod.eps fig16.eps # fig14.eps
cp ../realisticr.eps fig17.eps # fig15.eps


for i in *.eps; do
  echo $i
  m2u $i
  rm -f $i.orig
  epstopdf --outfile=`echo $i | sed -e 's/.eps//'`.pdf $i
  convert -density 150x150 `echo $i | sed -e 's/.eps//'`.pdf `echo $i | sed -e 's/.eps//'`.gif
  convert `echo $i | sed -e 's/.eps//'`.gif `echo $i | sed -e 's/.eps//'`.png
  convert -quality 72 `echo $i | sed -e 's/.eps//'`.png `echo $i | sed -e 's/.eps//'`.jpg
  jpeg2ps -h `echo $i | sed -e 's/.eps//'`.jpg > `echo $i | sed -e 's/.eps//'`.eps
done
cp ../band_pop_traj_layoutr.pdf fig11.pdf
convert -density 150x150 fig11.pdf fig11.gif
convert -crop 1275x1650-310+250 fig11.gif fig11.png
convert -quality 73 fig11.png fig11.jpg
jpeg2ps -h fig11.jpg > fig11.eps

#for i in fig*.pdf; do
#  head -n 1 $i > tmp.pdf
#  gs -sDEVICE=bbox -dNOPAUSE -dBATCH $i 2>> tmp.pdf 1>/dev/null 
#  tail -n $(( `wc -l $i | perl -pe 's/\S+$//'` - 1 )) $i >> tmp.pdf
#  mv -f tmp.pdf $i
#done
#  head -n 1 fig1.pdf > tmp.pdf
#  grep BoundingBox fig1.eps >> tmp.pdf
#  tail -n $(( `wc -l fig1.pdf | perl -pe 's/\S+$//'` - 1 )) fig1.pdf >> tmp.pdf
#  mv -f tmp.pdf fig1.pdf

cp ../ac.bib ./ac.bib
perl -pe 'if($c==""){$c=1;}if (/^\s*\\includegraphics/) {if (s/\{(\S+).eps/\{fig$c.eps/) {$c++;}}' < ../ac.tex > ./ac.tex
perl -pe 's/^\s*\\includegraphics\[scale=0.5\]{fig(\d+).eps}/     \\includegraphics[scale=0.41]{fig$1.eps}/' < ./ac.tex > ./ac.tex.tmp
perl -pe 's/^\s*\\includegraphics\[scale=0.41\]{fig1.eps}/     \\includegraphics[scale=0.52]{fig1.eps}/' < ./ac.tex.tmp > ./ac.tex
perl -pe 's/^\s*\\includegraphics\[scale=0.41\]{fig11.eps}/     \\includegraphics[scale=0.41]{fig11.eps}/' < ./ac.tex > ./ac.tex.tmp
mv -f ac.tex.tmp ac.tex
latex ac.tex &&\
bibtex ac.aux &&\
latex ac.tex &&\
bibtex ac.aux &&\
latex ac.tex 
latex ac.tex 
dvips -o -Pcmz -tletter ac.dvi &&\
ps2pdf ac.ps

rm *.aux *.blg *.log *.dvi *.ps *.png *.gif *.jpg fig*.pdf



